Structured Receptive Fields in CNNs

Learning powerful feature representations with CNNs is hard when training data are limited. Pre-training is one way to overcome this, but it requires large datasets sufficiently similar to the target domain. Another option is to design priors into the model, which can range from tuned hyperparameters to fully engineered representations like Scattering Networks. We combine these ideas into structured receptive field networks, a model which has a fixed filter basis and yet retains the flexibility of CNNs. This flexibility is achieved by expressing receptive fields in CNNs as a weighted sum over a fixed basis which is similar in spirit to Scattering Networks. The key difference is that we learn arbitrary effective filter sets from the basis rather than modeling the filters. This approach explicitly connects classical multiscale image analysis with general CNNs. With structured receptive field networks, we improve considerably over unstructured CNNs for small and medium dataset scenarios as well as over Scattering for large datasets. We validate our findings on ILSVRC2012, Cifar-10, Cifar-100 and MNIST. As a realistic small dataset example, we show state-of-the-art classification results on popular 3D MRI brain-disease datasets where pre-training is difficult due to a lack of large public datasets in a similar domain.

==> rfnn_final - update/sections/abs.tex <==
 \begin{abstract}

-Deep representation learning suffers from poor data efficiency. One way to deal with this is the incorporation of priors into the model, either through transfer learning or by design. We introduce structured receptive field networks that focus on the latter by restricting the classes of functions CNN-filters can effectively learn. In such a network, each filter's weights are the eigenvalues of a decomposition onto a linear combination of a complete set of basis functions. The type and order of basis represents the prior on the functions being learned. We show that Gaussian derivatives constitute a particularly suitable basis when applying structured receptive field networks on image data as they explicitly link multiscale feature analysis and reasoning to the concept of CNNs. The notion of a fixed basis is similar in spirit to Scattering Networks, while the key difference is that we learn arbitrary effective filter sets from a basis end-to-end rather than modelling them explicitly as Scattering requires. With the structured version of CNNs, we improve considerably over the original models for small dataset scenarios as well as over Scattering for large datasets. We achieve state-of-the-art classification results on a popular 3D MRI brain-disease dataset as an example of a domain where transfer learning is difficult due to a lack of large public datasets in a similar domain.

+Deep representation learning suffers from poor data efficiency~\jvg{I still do not like this. Maybe the ML people like to be vague, I prefer our old 'Where CNNs are powerful for the classification of images when ample data are available, we insert structured receptive fields in CNNs to train them with less image data.'}. One way to deal with this is the incorporation of priors into the model, either through transfer learning~\jvg{why relevant? Side track? Remove?} \jvg{Ok, you want to use it at the end, then I would advise to spend 1 sentence about pre-training, I also prefer the term 'pre-training', since it focuses on the network, while transfer learning can be some other module} or by design~\jvg{Here Scattering should be mentioned; some emphasis on pre-training some on Scattering}. \jvg{Sentence does not connect to the next:} We introduce structured receptive field networks that focus on the latter \jvg{motivation for reading comes too late: make it clear from the beginning why I am reading this. Please do not use 'latter' you force the reader to keep both of them in mind, or you force him to go back and read the same text again: neither options are good. Try to avoid reference-words such as 'latter'} by restricting the classes of functions CNN-filters can effectively learn~\jvg{'classes of function' is vague and not precise. Do we refer to classes of functions in the paper? It seems a Taylor series can approximate any function. So, do we back-up this claim with theory or results in the paper? If not then I would remove this. Why not introduce Gaussian filters without such a risky 'side-step'?}. In such a network~\jvg{Can you end the previous sentence so it ends with the 'network'? Then the 2 sentences will flow better eg: 'We add prior information in the form of structured Gaussian filters, forming a structured receptive field network' Not saying this sentence is the best, but it flows naturally to the next. }, each filter's weights are the eigenvalues of a decomposition onto a linear combination of a complete set of basis functions~\jvg{This may be correct, but it is not clear nor easy to read. What happened to the linear combination of Gaussian basis functions? Why postpone clarity so long?}. The type and order of basis represents the prior on the functions being learned~\jvg{Sentence has no goal. Remove?}. We show that Gaussian derivatives constitute a particularly suitable basis when applying structured receptive field networks on image data as they explicitly link multiscale feature analysis~\jvg{what is this? Not introduced why this is needed. Scale space and its benefits should be introduced before} and reasoning~\jvg{it adds 'reasoning'? like memory networks? please pick one: analysis or reasoning, but best not to overclaim} to the concept of \jvg{remove: 'to the concept of'} CNNs. The notion of \jvg{remove 'The notion of'} a fixed basis is similar in spirit to Scattering Networks, while the key difference is that we learn arbitrary effective filter sets from a basis end-to-end \jvg{I see no added contribution from the term 'end-to-end'} rather than modelling them explicitly as Scattering requires. With the structured version of CNNs \jvg{Its good to be consistent with new terminology: 'with structured receptive field networks'}, we improve considerably over the original \jvg{similar unstructured?} models for small dataset scenarios~\jvg{yes, why not call it data-efficient? ;) just kidding, i like small datasets, but I would prefer to consistently call it small datasets from the start} as well as over Scattering for large datasets. \jvg{Start the following sentence with 'as an example of ', that way the reader gets the relevant sentence-connection information directly} We achieve state-of-the-art classification results on a popular 3D MRI brain-disease dataset as an example of a domain where transfer learning is difficult due to a lack of large public datasets in a similar domain. \jvg{This is important. So, earlier I would spend 1 sentence to pre-training and one on Scattering}

 \end{abstract}

==> rfnn_final - update/sections/abstract.tex <==
 \begin{abstract}
Learning powerful feature representations with CNNs is hard when training data are limited. Pre-training is one way to overcome this, but it requires large datasets sufficiently similar to the target domain. Another option is to design priors into the model, which can range from tuned hyperparameters to fully engineered representations like Scattering Networks. We combine these ideas into structured receptive field networks, a model which has a fixed filter basis and yet retains the flexibility of CNNs. This flexibility is achieved by expressing receptive fields in CNNs as a weighted sum over a fixed basis which is similar in spirit to Scattering Networks. The key difference is that we learn arbitrary effective filter sets from the basis rather than modeling the filters. This approach explicitly connects classical multiscale image analysis with general CNNs. With structured receptive field networks, we improve considerably over unstructured CNNs for small and medium dataset scenarios as well as over Scattering for large datasets. We validate our findings on ILSVRC2012, Cifar-10, Cifar-100 and MNIST. As a realistic small dataset example, we show state-of-the-art classification results on popular 3D MRI brain-disease datasets where pre-training is difficult due to a lack of large public datasets in a similar domain.
 \end{abstract}

==> rfnn_final - update/sections/exp.tex <==
documentclass[../rfnn.tex]{subfiles}
\begin{document} 
\section{Experiments}


The experimental section focuses on gaining insight into the proposed architecture by investigation of its strengths and weaknesses. The experiments are partitioned into four parts. i) We show insight in the proposed model to motivate design choices; ii) we show that our model combines the strengths of Scattering and CNNs; iii) we show structured receptive fields aid classification performance when artificially limiting training data; iv) we show a 3D version of our model outperforms the state-of-the-art on a small brain MRI classification dataset where large pre-training datasets are not available. We use the Caffe library~\cite{jia2014caffe} and Theano~\cite{bastien2012theano} where we added RFNN as a separate module.

\subsection{Experiment 1: Model insight}

The RFNN used in this section is the RF version of the Network in Network (RFNiN) introduced in section 3.3. We gain insight into the model by evaluating the scale and order of the basis filters. In addition we analyze the performance compared to the standard Network in Network (NiN)~\cite{linArxiv13NetwInNetw} and Alexnet~\cite{krizhevskyNIPS12imagenet}. We further highlight that our proposed model is not merely a change in architecture by refactorizing the NiN model in such a way that it has the identical architecture as our proposed model. To allow overnight experiments we use the 100 largest classes of the ILSVRC2012 ImageNet classification challenge~\cite{russakovskyIJCV14imagenet}. Selection is done by folder size, as more than 100 classes have 1,300 images in them, yielding a dataset size of 130,000 images. This is a real-world medium sized dataset in a domain where CNNs excel. 

\textbf{Experimental setup}. The Network in Network (NiN) model and our Structured Receptive Field Network in Network (RFNiN) model are based on the training definitions provided by the Caffe model zoo~\cite{jia2014caffe}. Training is done with the standard procedure on Imagenet. We use stochastic gradient descent, a momentum of 0.9, a weight decay of 0.0005 and a batch size of 64 images. The images are re-sized to 256x256, mirrored during training and the dataset mean is subtracted. The base learning rate was decreased by a factor of 10, according to the reduction from 1000 to 100 classes, to ensure proper scaling of the weight updates. We decreased it by a factor of 10 after 50,000 iterations. The networks were trained for 100,000 iterations. Results are computed as the mean classification accuracy on the validation set. \\

\begin{table}
\begin{center}
\begin{tabular}{@{}llll@{}}\toprule
\multicolumn{4}{l}{ILSVRC2012-100 Subset}\\ \midrule

Method & Top-1 & 2DFilters & $\#$Params \\ \midrule    %& Accuracy LR 0.01 \\

RFNiN $1^{st}$-order & 44.83\%  &$12$ & 1.8M \\
RFNiN $2^{nd}$-order & 61.24\%  &$24$ & 3.4M \\
RFNiN $3^{rd}$-order & 63.64\%  &$40$ & 5.5M\\
RFNiN $4^{th}$-order & 62.92\%  &$60$ & 8.1M\\
RFNiN-Scale $1^{st}$-order &  57.21\% &$24$ & 2.2M\\
RFNiN-Scale $2^{nd}$-order &  67.56\% &$54$& 4.2M\\
RFNiN-Scale $3^{rd}$-order &  \textbf{69.65\%} &$94$ & 6.8M\\ 
RFNiN-Scale $4^{th}$-order &  68.95\% &$144$   & 10.1M\\
\midrule   
Network in Network & 67.30\% &$520k$ &  8.2M\\
Alexnet & 54.86\% &$370k$ & 60.0M\\  \bottomrule
%\hline\hline
%Alexnet \textit{Pre-train} & 71.99 / 64.88  \% &$3,689,28$ & \\
%Network in Network \textit{Pre-train} &  /  64.01 \% &$516,384$ &  \\
\end{tabular}
\end{center}
\caption{\textbf{Results on 100 Biggest ILSVRC2012 Classes:} The table shows RFNiN with 1st, 2nd, 3rd and 4th order filters in the whole network. Row 1-4 are applying basis filters in all layers on a scale of $\sigma$=1. RFNiN-scale in row 5-8 applies basis filters on 4 scales, where $\sigma$=1,2,4,8. The results show that a $3^{rd}$ order basis is sufficient while incorporating scale into the network gives a big gain in performance. The RFNiN outperforms the same Network in Network architecture while having only a fraction of filters in total.}
\label{tab:ILSVRC100}
\end{table}


\textbf{Filter basis order}. 
In the table~\ref{tab:ILSVRC100}, the first four rows show the result of RFNiN architectures with a 1st to 4th order of the Gaussian derivative basis filter set comprised of 12 to 60 individual Gaussian filters in all layers of the network. In these experiments the value of $\sigma$=1, fixed for all filters and all layers. Comparing first to third order filter basis in table~\ref{tab:ILSVRC100}, we conclude that third order is sufficient, outperforming first and second order as predicted by scale space theory~\cite{koenderinkBioCyb87localGeoInVisSys} and Scattering Networks~\cite{brunaTPAMI13scattering} as third order filters are capable of computing rotations of second and third order filters, also used in the scattering network. The fourth order does not add any more gain. 


\textbf{Filter scale}. The \emph{RFNiN-Scale} entries of table~\ref{tab:ILSVRC100} show the classification result upto fourth order now with 4 different scales, $\sigma$=1, 2, 4, 8 for the lowest layer, $\sigma$=2, 4, 8 for the second layer, $\sigma$=4, 8 for the third, and $\sigma$=8 for the fourth. This implies that the basis filter set expands from 24 up to 144 filters in total in the network. Comparing the use of single scale filters in the network or copies of the filters with varying scale indicates that a considerable gain can be achieved by including filters with different scales. This observation is supported by Scattering~\cite{brunaTPAMI13scattering}, showing that the multiple scales can directly be extracted from the first layer on. In fact normal CNNs are also capable of similar behaviour, as positive valued low-pass filter's feature maps are not affected by rectifier nonlinearities~\cite{sifreCVPR13rotScat}. Thus scale can directly be computed from the first layer onwards, which yields a much smaller set of filters and convolutions needed in the higher layers.


\begin{figure}
\includegraphics[width=.5\textwidth, left]{alphas_all_layers_imagenet_beta.png}
\caption{Mean of filter weights and variances per layer for 15 basis filters, as trained on ILSVRC2012 100 subset. Note that the lower order filters have the highest weights and are most informative. Zero-order filters are most effective in higher layers for combinations of lower responses.
\label{fig:alphaPerLayer}}
\end{figure}


\textbf{Analysis of network layers}.
For the network RFNiN 4th-order Figure~\ref{fig:alphaPerLayer} provides an overview of the range of basis weights per effective filter in all layers, where the x-axis indexes the spatial derivative index and y-axis the mean value of weights per layer over all effective filter kernels. The figure indicates that first order filters have the highest weights in all layers. Furthermore zero order filters have relatively high weights in higher layers, which hints to passing on incoming features, needed for combinations of different features. Some of the learned filters are also visualized in \ref{fig:visLayers} to illustrate their expressiveness.

\textbf{Comparison to Network in Network}.
The champion RFNiN in table~\ref{tab:ILSVRC100} slightly outperforms the Network in Network with the same setting and training circumstances while only having 94 instead 510,000 spatial filters in the network in total. This shows that our basis representation is sufficient and yields a more compact representation than the filters learned by the standard Network in Network. 

\textbf{Refactorize Network in Network}.
To illustrate that our proposed model is not merely a change in architecture we compare to a third architecture. We remove the Gaussian basis and we factorize the NiN such that it becomes identical to RFNiN. Both have almost the same number of parameters, but the NiN-factorize has a freely learnable basis. Factorizing only the first layer and leaving the rest of the network as in the original NiN shows that a Gaussian basis is superior to a learned basis. When factorizing all layers, RFNiN-Scale $3^\text{rd}$-order results are superior by far to the identical NiN-factorize All Layers (see table~\ref{tab:refactor}).

\begin{table}[htb]
\begin{center}
\begin{tabular}{@{}lll|l@{}}
\multicolumn{4}{l}{}\\ \midrule 
\multicolumn{3}{l}{ILSVRC2012-100 Refactorize NiN}\\ \midrule
Model&Basis&$\#$Params&Top-1\\ \midrule 
NiN-refactor Layer 1&Free&7.47M&64.10\%\\
RFNiN-refactor Layer 1&Gauss&7.47M&68.63\%\\ \midrule
NiN-refactor All Layers&Free&6.87M&38.02\%\\
RFNiN-Scale $3^\text{rd}$-order&Gauss&6.83M&69.65\%\\  \bottomrule
\end{tabular}
\caption{Classification experiment on ILSVRC2012-100 to illustrate influence of factorization on performance. The results show that indeed the advantage of the Gaussian basis is substantial and our results are not merely due to a change in architecture.}
\label{tab:refactor}
\end{center}
\end{table}



\subsection{Experiment 2: Scattering and RFNNs}



\textbf{Small dataset domain}. We compare a RFNN to scattering in classification on reduced training sizes of the MNIST dataset. This is the domain where scattering outperforms standard CNNs~\cite{brunaTPAMI13scattering}. To demonstrate equal quality of RFNN compared with Scattering, we reduce the number of training samples when training on MNIST as done in~\cite{brunaTPAMI13scattering}.
The network and training parameters used in this section are the same as in~\cite{zeiler2013stochastic}. The RFNN contains of 3 layers with a basis of 10 filters and a $sigma$=1 each. Scale is not considered in this case, as MNIST is only on one fixed scale. Each basis layer is followed by a layer of $\alpha$=64 parameters that linearly re-combine the basis filters outcomes. As comparison we re-implement the same model as a plain CNN and plot it in the same figure, to assure that our performance is not due to the model architecure itself. The CNN state of the art and Scattering results on the task are taken from~\cite{brunaTPAMI13scattering,ranzato2007unsupervised}.

Results are shown in Figure~\ref{fig:MNIST}, each number is averaged over 3 runs. For the experiment on MNIST the gap between the CNNs and networks with pre-defined filters increases when training data is reduced, while RFNN and Scattering perform on par even at the smallest sample size.

\textbf{Large complex domain}.
We compare against Scattering on the Cifar-10 and Cifar-100 datasets, as achieved by the recently introduced Deep Roto-Translation Scattering approach~\cite{sifreCVPR13rotScat}, a powerful variant of the Scattering approach. This is a domain where CNNs excel and learning of complex image variabilities is key.

The RFNN is again a variant of the standard NiN for Cifar-10. It is similar to the model in experiment 1, just that it has one basis layer, two 1x1 convolution layers and one pooling layer less and the units in the 1x1 convolution layers are 192 in the whole network. Furthermore we show performance of the state-of-the-art recurrent convolutional networks(RCNNs)~\cite{liang2015recurrent} for comparison. 

The results in Table~\ref{tab:SCAT} show a considerable improvement on Cifar-10 and Cifar-100 when comparing RFNN to Roto-Translation Scattering \cite{sifreCVPR13rotScat}, which was designed specifically for this dataset. RCNNs performance is considerably higher as they follow a different approach to which structured receptive fields can also be applied if desired. \\

\textbf{RFNNs are robust to dataset size}.
From these experiments we conclude that RFNNs combine the best of both worlds. We outperform CNNs and compete with scattering when training data is limited as exemplified on subsets of MNIST. While we capture complex image variabilities beyond the capabilities of scattering representations as exemplified on the datasets Cifar-10 and Cifar-100.



\begin{table}
\centering
\begin{tabular}{lll}\midrule
Model & Cifar-10 & Cifar-100\\ \midrule
Roto-Trans Scattering & 82.30\% & 56.80\% \\
RFNiN & 86.31\% & 63.81\%\\ \bottomrule
%NiN (Caffe)&87.30\%&\%&-\%\\ 
%NiN~\cite{}&89.59\%&64.32\%&99.53\%\\
RCNN&91.31\%&68.25\%\\
\bottomrule
\end{tabular}
\caption{Comparison against Scattering on a large complex domain. The best results is given by RCNN, yet RFNN outperforms the Scattering.}
\label{tab:SCAT}
\end{table}

\subsection{Experiment 3: Limiting Datasize}


To demonstrate the effectiveness of the RF variant compared in the Network in Network, we reduce the number of classes in the 100-class ILSVRC2012-dataset from 100 to 10, resulting in a reduction of the total number of images on which the network was trained from 130k to 13k.

The results in Table~\ref{tab:imnetSubsets} show that the RFNN performance is better relatively speaking when the number of samples decreases compared to CNNs in natural images and stays as robust as scattering in the domain where Scattering excels and CNNs are weak. 
For the 13,000 ILSVRC2012-10 image dataset the gap with the Network in Network architecture has increased to 8.0\% from 2.4\% for the 130,000 images. This supports our aim that RF Network in Networks are more effectively learning from image data compared to the standard Network in Network.


\begin{table}
\begin{center}
\begin{tabular}{@{}llll@{}}\midrule
ILSVRC2012 Subset:&1000-class&100-class &10-class\\ \midrule %& ILSVRC2012-2\\ \midrule
RFNiN-Scale $3^{rd}$-order&55.91\%&69.65\%&85.00\%  \\
Network in Network&58.21\%&67.30\%&76.97\% \\ \midrule
\end{tabular}
\end{center}
\caption{Taking subsets of ImageNet. The gap between RFNNs and CNNs increases for fewer classes.}
\label{tab:imnetSubsets}
\end{table}


\begin{figure}
\includegraphics[width=0.5\textwidth, center]{mnist.eps}
\caption{Classification performance of the scattering network on various subsets of the MNIST dataset. In comparison the state of the art CNN-A from the literature on a subset of 300 samples. RFNN denotes our receptive field network, with the same architecture as CNN-B. Both are shown, to illustrate that good performance of the RFNN is not due to the CNN architecture, but due to RFNN decomposition. Our RFNN performs on par with Scattering, substantially outperforming CNN's on random MNIST subsets.}
\label{fig:MNIST}
\end{figure}


% The second part of the experiments is concerned with comparison to the scattering approach to show, that we outperform it on very small MNIST subsets as an example of very small non-natural image datasets where the scattering network has been shown to be state of the art~\cite{brunaTPAMI13scattering}, while we also perform better on the more challenging datasets Cifar-10/100, shown in [REF].
 
 
%We compare our approach to scattering networks on three datasets. We use multiple averaged runs on a tiny subset of MNIST to illustrate our ability to tackle small data non-natural image problems. On this problem scattering is de-facto state of the art. Furthermore we compare on two more challenging benchmarks, Cifar-10 and Cifar-100.

\subsection{Experiment 4: 3D Classification}

%We do two experiments on medical images, to show the value of our approach for images where pre-training doesn't work (2D Bone texture), or is simply not possible (3D Brain Scans).

 
We apply a RFNN to 3D brain scan classification for Alzheimer's~\cite{cuingnet2011automatic}, a domain where training data is notoriously small and no big open access databases in a similar domain exist for pre-training. \\

We use a 3 layer RFNiN, with a basis of order 10 in 3 scales $\sigma$=1,4,16. This time more extremely spaced, as the brains are always centered and have been normalized to MNI space with FSL library~\cite{jenkinson2012fsl}. Each basis layer is followed by one 1x1 convolution layer. Having 128 units in layer 1, 96 units in layer 2 and 64 units in layer 3. Global average pooling is applied to the final feature maps. The network has been implemented in the Theano library~\cite{bastien2012theano}.

The results are in Table~\ref{tab:brains}. We outperform the state-of-the-art, including a 3D CNN. The same 3 layer NiN as our RFNiN model does not converge on the dataset and gives random predictions. Thus we show our model is effective when data is scarce.


\begin{table}
\begin{center}
\begin{tabular}{@{}llll@{}}\toprule
Method&Accuracy&TPR&SPC\\ \midrule
%3D-RFNN A&99.32\%& &\\
3D-RFNiN (ours)&\textbf{97.79\%}& \textbf{97.14\%}& \textbf{98.78\%} \\
%3D-CNN A&98.79\%& &\\
%3D-CNN B&(Chance)\%& &\\
3D-CNN~\cite{DBLP:journals/corr/PayanM15}&95.70\%&-&-\\
NIB~\cite{gupta2013natural}&94.74\%&95.24\%&94.26\%\\
ICA~\cite{yang2011independent}&80.70\%&81.90\%&79.50\%\\
Voxel-Direct-D-gm~\cite{cuingnet2011automatic}&-&81.00\%&95.00\%\\ \midrule
3D-NiN (our baseline)&84.21\%& -\%& -\% \\
\midrule
\end{tabular}
\end{center}
\caption{Results on training with 150 brain MRI images of the ADNI standard benchmark. RFNNs outperform all published results. Reported is classification accuracy, true positive rate and specificity on the test set.}
\label{tab:brains}
\end{table}

\begin{table}
\begin{center}
\begin{tabular}{@{}llll@{}}\midrule
Method&Accuracy&EER\\ \midrule
3D-RFNiN (ours)&\textbf{87.67\%}& \textbf{-}& \textbf{-} \\
Local SVM~\cite{chen2014detecting}&74.10\%&-&-\\
FBM~\cite{toews2010feature}&-&70.00\%&-\\
Voxel-Direct-D-gm~\cite{cuingnet2011automatic}&-&-\%&-\%\\
\bottomrule
\end{tabular}
\end{center}
\caption{Results of training on the OASIS AD-126 dataset described in~\cite{toews2010feature}. Training has been done by .....}
\label{tab:brains}
\end{table}


%\begin{table}
%\begin{center}
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
%\hline
%RFNN based on NiN  \\
%Basis& 1x1Conv& ReLU& 1x1Conv& ReLU& MaxPool& Basis& 1x1Conv& ReLU& 1x1Conv& ReLU& MaxPool& Basis& 1x1Conv& ReLU& 1x1Conv& ReLU& MaxPool& Basis& 1x1Conv& ReLU& %1x1Conv& ReLU& Global Pool
%\hline
%\end{tabular}
%\end{center}
%\caption{RFNN architecture used}
%\end{table}


%\begin{table}
%\begin{center}
%\begin{tabular}{|l|l|}
%\hline
%Filters in Layer 1 & Top-1  \\%& Accuracy LR 0.01 \\
%\hline\hline
%Network in Network-96 & 56.85\% \\
%Network in Network-15 & 55.62\%  \\
%RFNN $1^{st}$-order & 54.16\% \\
%RFNN $2^{nd}$-order & 55.28\% \\
%RFNN $3^{rd}$-order & 57.60\% \\
%RFNN $4^{th}$-order & 70.22\%  \\
%\hline
%\end{tabular}
%\end{center}
%\caption{Shows orders for first layer basis. These results were trained with RMSprop due to the different learning rates necessary per layer.}
%\end{table}






%\begin{table}
%\begin{center}
%\begin{tabular}{@{}lll@{}}\toprule
%Method & Top-1 & \# of Parameters \\ \midrule
%RFNN scale=1 & running\% \\
%RFNN scale=2 & running\% \\
%RFNN scale=3 & ??\% \\
%RFNN scale=4 & ??\% \\  \bottomrule
%\end{tabular}
%\end{center}
%\caption{Table 1c RFNN with increased scale, up to scale 4 (5 if time). This affects all layers, as there is no reason for scale only to be extracted in layer 1, frequency decreasing paths can be ommited, thus higher layer have lesser sigmas -> 4*10h=50h}
%\end{table}





%\begin{table}
%\begin{center}
%\begin{tabular}{|l|c|c|c|}
%\hline
%Method & Top-1 & Top-5 \\
%\hline\hline
%RFNN  & \% & &\\
%Alexnet  & \% & &\\
%NiN  & \% & &\\
%\hline
%\end{tabular}
%\end{center}
%\caption{Full Imagenet}
%\end{table}







%\begin{figure}
%\includegraphics[width=0.5\textwidth, right]{filters_ordered_L1_beta.png}
%\caption{Effective filters learned by the network in Layer 1, ordered by highest energy per order and rotation. Higher scales are normalized for visualization by multiplying them with sigma. 
%\label{fig:filters}}
%\end{figure}






\end{document}


==> sections/abs.tex <==
 \begin{abstract}

-Deep representation learning suffers from poor data efficiency. One way to deal with this is the incorporation of priors into the model, either through transfer learning or by design. We introduce structured receptive field networks that focus on the latter by restricting the classes of functions CNN-filters can effectively learn. In such a network, each filter's weights are the eigenvalues of a decomposition onto a linear combination of a complete set of basis functions. The type and order of basis represents the prior on the functions being learned. We show that Gaussian derivatives constitute a particularly suitable basis when applying structured receptive field networks on image data as they explicitly link multiscale feature analysis and reasoning to the concept of CNNs. The notion of a fixed basis is similar in spirit to Scattering Networks, while the key difference is that we learn arbitrary effective filter sets from a basis end-to-end rather than modelling them explicitly as Scattering requires. With the structured version of CNNs, we improve considerably over the original models for small dataset scenarios as well as over Scattering for large datasets. We achieve state-of-the-art classification results on a popular 3D MRI brain-disease dataset as an example of a domain where transfer learning is difficult due to a lack of large public datasets in a similar domain.

+Deep representation learning suffers from poor data efficiency~\jvg{I still do not like this. Maybe the ML people like to be vague, I prefer our old 'Where CNNs are powerful for the classification of images when ample data are available, we insert structured receptive fields in CNNs to train them with less image data.'}. One way to deal with this is the incorporation of priors into the model, either through transfer learning~\jvg{why relevant? Side track? Remove?} \jvg{Ok, you want to use it at the end, then I would advise to spend 1 sentence about pre-training, I also prefer the term 'pre-training', since it focuses on the network, while transfer learning can be some other module} or by design~\jvg{Here Scattering should be mentioned; some emphasis on pre-training some on Scattering}. \jvg{Sentence does not connect to the next:} We introduce structured receptive field networks that focus on the latter \jvg{motivation for reading comes too late: make it clear from the beginning why I am reading this. Please do not use 'latter' you force the reader to keep both of them in mind, or you force him to go back and read the same text again: neither options are good. Try to avoid reference-words such as 'latter'} by restricting the classes of functions CNN-filters can effectively learn~\jvg{'classes of function' is vague and not precise. Do we refer to classes of functions in the paper? It seems a Taylor series can approximate any function. So, do we back-up this claim with theory or results in the paper? If not then I would remove this. Why not introduce Gaussian filters without such a risky 'side-step'?}. In such a network~\jvg{Can you end the previous sentence so it ends with the 'network'? Then the 2 sentences will flow better eg: 'We add prior information in the form of structured Gaussian filters, forming a structured receptive field network' Not saying this sentence is the best, but it flows naturally to the next. }, each filter's weights are the eigenvalues of a decomposition onto a linear combination of a complete set of basis functions~\jvg{This may be correct, but it is not clear nor easy to read. What happened to the linear combination of Gaussian basis functions? Why postpone clarity so long?}. The type and order of basis represents the prior on the functions being learned~\jvg{Sentence has no goal. Remove?}. We show that Gaussian derivatives constitute a particularly suitable basis when applying structured receptive field networks on image data as they explicitly link multiscale feature analysis~\jvg{what is this? Not introduced why this is needed. Scale space and its benefits should be introduced before} and reasoning~\jvg{it adds 'reasoning'? like memory networks? please pick one: analysis or reasoning, but best not to overclaim} to the concept of \jvg{remove: 'to the concept of'} CNNs. The notion of \jvg{remove 'The notion of'} a fixed basis is similar in spirit to Scattering Networks, while the key difference is that we learn arbitrary effective filter sets from a basis end-to-end \jvg{I see no added contribution from the term 'end-to-end'} rather than modelling them explicitly as Scattering requires. With the structured version of CNNs \jvg{Its good to be consistent with new terminology: 'with structured receptive field networks'}, we improve considerably over the original \jvg{similar unstructured?} models for small dataset scenarios~\jvg{yes, why not call it data-efficient? ;) just kidding, i like small datasets, but I would prefer to consistently call it small datasets from the start} as well as over Scattering for large datasets. \jvg{Start the following sentence with 'as an example of ', that way the reader gets the relevant sentence-connection information directly} We achieve state-of-the-art classification results on a popular 3D MRI brain-disease dataset as an example of a domain where transfer learning is difficult due to a lack of large public datasets in a similar domain. \jvg{This is important. So, earlier I would spend 1 sentence to pre-training and one on Scattering}

 \end{abstract}

==> sections/exp.tex <==
documentclass[../rfnn.tex]{subfiles}
\begin{document} 
\section{Experiments}


The experimental section focuses on gaining insight into the proposed architecture by investigation of its strengths and weaknesses. The experiments are partitioned into four parts. i) We show insight in the proposed model to motivate design choices; ii) we show that our model combines the strengths of Scattering and CNNs; iii) we show structured receptive fields aid classification performance when artificially limiting training data; iv) we show a 3D version of our model outperforms the state-of-the-art on a small brain MRI classification dataset where large pre-training datasets are not available. We use the Caffe library~\cite{jia2014caffe} and Theano~\cite{bastien2012theano} where we added RFNN as a separate module.

\subsection{Experiment 1: Model insight}

The RFNN used in this section is the RF version of the Network in Network (RFNiN) introduced in section 3.3. We gain insight into the model by evaluating the scale and order of the basis filters. In addition we analyze the performance compared to the standard Network in Network (NiN)~\cite{linArxiv13NetwInNetw} and Alexnet~\cite{krizhevskyNIPS12imagenet}. We further highlight that our proposed model is not merely a change in architecture by refactorizing the NiN model in such a way that it has the identical architecture as our proposed model. To allow overnight experiments we use the 100 largest classes of the ILSVRC2012 ImageNet classification challenge~\cite{russakovskyIJCV14imagenet}. Selection is done by folder size, as more than 100 classes have 1,300 images in them, yielding a dataset size of 130,000 images. This is a real-world medium sized dataset in a domain where CNNs excel. 

\textbf{Experimental setup}. The Network in Network (NiN) model and our Structured Receptive Field Network in Network (RFNiN) model are based on the training definitions provided by the Caffe model zoo~\cite{jia2014caffe}. Training is done with the standard procedure on Imagenet. We use stochastic gradient descent, a momentum of 0.9, a weight decay of 0.0005 and a batch size of 64 images. The images are re-sized to 256x256, mirrored during training and the dataset mean is subtracted. The base learning rate was decreased by a factor of 10, according to the reduction from 1000 to 100 classes, to ensure proper scaling of the weight updates. We decreased it by a factor of 10 after 50,000 iterations. The networks were trained for 100,000 iterations. Results are computed as the mean classification accuracy on the validation set. \\

\begin{table}
\begin{center}
\begin{tabular}{@{}llll@{}}\toprule
\multicolumn{4}{l}{ILSVRC2012-100 Subset}\\ \midrule

Method & Top-1 & 2DFilters & $\#$Params \\ \midrule    %& Accuracy LR 0.01 \\

RFNiN $1^{st}$-order & 44.83\%  &$12$ & 1.8M \\
RFNiN $2^{nd}$-order & 61.24\%  &$24$ & 3.4M \\
RFNiN $3^{rd}$-order & 63.64\%  &$40$ & 5.5M\\
RFNiN $4^{th}$-order & 62.92\%  &$60$ & 8.1M\\
RFNiN-Scale $1^{st}$-order &  57.21\% &$24$ & 2.2M\\
RFNiN-Scale $2^{nd}$-order &  67.56\% &$54$& 4.2M\\
RFNiN-Scale $3^{rd}$-order &  \textbf{69.65\%} &$94$ & 6.8M\\ 
RFNiN-Scale $4^{th}$-order &  68.95\% &$144$   & 10.1M\\
\midrule   
Network in Network & 67.30\% &$520k$ &  8.2M\\
Alexnet & 54.86\% &$370k$ & 60.0M\\  \bottomrule
%\hline\hline
%Alexnet \textit{Pre-train} & 71.99 / 64.88  \% &$3,689,28$ & \\
%Network in Network \textit{Pre-train} &  /  64.01 \% &$516,384$ &  \\
\end{tabular}
\end{center}
\caption{\textbf{Results on 100 Biggest ILSVRC2012 Classes:} The table shows RFNiN with 1st, 2nd, 3rd and 4th order filters in the whole network. Row 1-4 are applying basis filters in all layers on a scale of $\sigma$=1. RFNiN-scale in row 5-8 applies basis filters on 4 scales, where $\sigma$=1,2,4,8. The results show that a $3^{rd}$ order basis is sufficient while incorporating scale into the network gives a big gain in performance. The RFNiN outperforms the same Network in Network architecture while having only a fraction of filters in total.}
\label{tab:ILSVRC100}
\end{table}


\textbf{Filter basis order}. 
In the table~\ref{tab:ILSVRC100}, the first four rows show the result of RFNiN architectures with a 1st to 4th order of the Gaussian derivative basis filter set comprised of 12 to 60 individual Gaussian filters in all layers of the network. In these experiments the value of $\sigma$=1, fixed for all filters and all layers. Comparing first to third order filter basis in table~\ref{tab:ILSVRC100}, we conclude that third order is sufficient, outperforming first and second order as predicted by scale space theory~\cite{koenderinkBioCyb87localGeoInVisSys} and Scattering Networks~\cite{brunaTPAMI13scattering} as third order filters are capable of computing rotations of second and third order filters, also used in the scattering network. The fourth order does not add any more gain. 


\textbf{Filter scale}. The \emph{RFNiN-Scale} entries of table~\ref{tab:ILSVRC100} show the classification result upto fourth order now with 4 different scales, $\sigma$=1, 2, 4, 8 for the lowest layer, $\sigma$=2, 4, 8 for the second layer, $\sigma$=4, 8 for the third, and $\sigma$=8 for the fourth. This implies that the basis filter set expands from 24 up to 144 filters in total in the network. Comparing the use of single scale filters in the network or copies of the filters with varying scale indicates that a considerable gain can be achieved by including filters with different scales. This observation is supported by Scattering~\cite{brunaTPAMI13scattering}, showing that the multiple scales can directly be extracted from the first layer on. In fact normal CNNs are also capable of similar behaviour, as positive valued low-pass filter's feature maps are not affected by rectifier nonlinearities~\cite{sifreCVPR13rotScat}. Thus scale can directly be computed from the first layer onwards, which yields a much smaller set of filters and convolutions needed in the higher layers.


\begin{figure}
\includegraphics[width=.5\textwidth, left]{alphas_all_layers_imagenet_beta.png}
\caption{Mean of filter weights and variances per layer for 15 basis filters, as trained on ILSVRC2012 100 subset. Note that the lower order filters have the highest weights and are most informative. Zero-order filters are most effective in higher layers for combinations of lower responses.
\label{fig:alphaPerLayer}}
\end{figure}


\textbf{Analysis of network layers}.
For the network RFNiN 4th-order Figure~\ref{fig:alphaPerLayer} provides an overview of the range of basis weights per effective filter in all layers, where the x-axis indexes the spatial derivative index and y-axis the mean value of weights per layer over all effective filter kernels. The figure indicates that first order filters have the highest weights in all layers. Furthermore zero order filters have relatively high weights in higher layers, which hints to passing on incoming features, needed for combinations of different features. Some of the learned filters are also visualized in \ref{fig:visLayers} to illustrate their expressiveness.

\textbf{Comparison to Network in Network}.
The champion RFNiN in table~\ref{tab:ILSVRC100} slightly outperforms the Network in Network with the same setting and training circumstances while only having 94 instead 510,000 spatial filters in the network in total. This shows that our basis representation is sufficient and yields a more compact representation than the filters learned by the standard Network in Network. 

\textbf{Refactorize Network in Network}.
To illustrate that our proposed model is not merely a change in architecture we compare to a third architecture. We remove the Gaussian basis and we factorize the NiN such that it becomes identical to RFNiN. Both have almost the same number of parameters, but the NiN-factorize has a freely learnable basis. Factorizing only the first layer and leaving the rest of the network as in the original NiN shows that a Gaussian basis is superior to a learned basis. When factorizing all layers, RFNiN-Scale $3^\text{rd}$-order results are superior by far to the identical NiN-factorize All Layers (see table~\ref{tab:refactor}).

\begin{table}[htb]
\begin{center}
\begin{tabular}{@{}lll|l@{}}
\multicolumn{4}{l}{}\\ \midrule 
\multicolumn{3}{l}{ILSVRC2012-100 Refactorize NiN}\\ \midrule
Model&Basis&$\#$Params&Top-1\\ \midrule 
NiN-refactor Layer 1&Free&7.47M&64.10\%\\
RFNiN-refactor Layer 1&Gauss&7.47M&68.63\%\\ \midrule
NiN-refactor All Layers&Free&6.87M&38.02\%\\
RFNiN-Scale $3^\text{rd}$-order&Gauss&6.83M&69.65\%\\  \bottomrule
\end{tabular}
\caption{Classification experiment on ILSVRC2012-100 to illustrate influence of factorization on performance. The results show that indeed the advantage of the Gaussian basis is substantial and our results are not merely due to a change in architecture.}
\label{tab:refactor}
\end{center}
\end{table}



\subsection{Experiment 2: Scattering and RFNNs}



\textbf{Small dataset domain}. We compare a RFNN to scattering in classification on reduced training sizes of the MNIST dataset. This is the domain where scattering outperforms standard CNNs~\cite{brunaTPAMI13scattering}. To demonstrate equal quality of RFNN compared with Scattering, we reduce the number of training samples when training on MNIST as done in~\cite{brunaTPAMI13scattering}.
The network and training parameters used in this section are the same as in~\cite{zeiler2013stochastic}. The RFNN contains of 3 layers with a basis of 10 filters and a $sigma$=1 each. Scale is not considered in this case, as MNIST is only on one fixed scale. Each basis layer is followed by a layer of $\alpha$=64 parameters that linearly re-combine the basis filters outcomes. As comparison we re-implement the same model as a plain CNN and plot it in the same figure, to assure that our performance is not due to the model architecure itself. The CNN state of the art and Scattering results on the task are taken from~\cite{brunaTPAMI13scattering,ranzato2007unsupervised}.

Results are shown in Figure~\ref{fig:MNIST}, each number is averaged over 3 runs. For the experiment on MNIST the gap between the CNNs and networks with pre-defined filters increases when training data is reduced, while RFNN and Scattering perform on par even at the smallest sample size.

\textbf{Large complex domain}.
We compare against Scattering on the Cifar-10 and Cifar-100 datasets, as achieved by the recently introduced Deep Roto-Translation Scattering approach~\cite{sifreCVPR13rotScat}, a powerful variant of the Scattering approach. This is a domain where CNNs excel and learning of complex image variabilities is key.

The RFNN is again a variant of the standard NiN for Cifar-10. It is similar to the model in experiment 1, just that it has one basis layer, two 1x1 convolution layers and one pooling layer less and the units in the 1x1 convolution layers are 192 in the whole network. Furthermore we show performance of the state-of-the-art recurrent convolutional networks(RCNNs)~\cite{liang2015recurrent} for comparison. 

The results in Table~\ref{tab:SCAT} show a considerable improvement on Cifar-10 and Cifar-100 when comparing RFNN to Roto-Translation Scattering \cite{sifreCVPR13rotScat}, which was designed specifically for this dataset. RCNNs performance is considerably higher as they follow a different approach to which structured receptive fields can also be applied if desired. \\

\textbf{RFNNs are robust to dataset size}.
From these experiments we conclude that RFNNs combine the best of both worlds. We outperform CNNs and compete with scattering when training data is limited as exemplified on subsets of MNIST. While we capture complex image variabilities beyond the capabilities of scattering representations as exemplified on the datasets Cifar-10 and Cifar-100.



\begin{table}
\centering
\begin{tabular}{lll}\midrule
Model & Cifar-10 & Cifar-100\\ \midrule
Roto-Trans Scattering & 82.30\% & 56.80\% \\
RFNiN & 86.31\% & 63.81\%\\ \bottomrule
%NiN (Caffe)&87.30\%&\%&-\%\\ 
%NiN~\cite{}&89.59\%&64.32\%&99.53\%\\
RCNN&91.31\%&68.25\%\\
\bottomrule
\end{tabular}
\caption{Comparison against Scattering on a large complex domain. The best results is given by RCNN, yet RFNN outperforms the Scattering.}
\label{tab:SCAT}
\end{table}

\subsection{Experiment 3: Limiting Datasize}


To demonstrate the effectiveness of the RF variant compared in the Network in Network, we reduce the number of classes in the 100-class ILSVRC2012-dataset from 100 to 10, resulting in a reduction of the total number of images on which the network was trained from 130k to 13k.

The results in Table~\ref{tab:imnetSubsets} show that the RFNN performance is better relatively speaking when the number of samples decreases compared to CNNs in natural images and stays as robust as scattering in the domain where Scattering excels and CNNs are weak. 
For the 13,000 ILSVRC2012-10 image dataset the gap with the Network in Network architecture has increased to 8.0\% from 2.4\% for the 130,000 images. This supports our aim that RF Network in Networks are more effectively learning from image data compared to the standard Network in Network.


\begin{table}
\begin{center}
\begin{tabular}{@{}llll@{}}\midrule
ILSVRC2012 Subset:&1000-class&100-class &10-class\\ \midrule %& ILSVRC2012-2\\ \midrule
RFNiN-Scale $3^{rd}$-order&55.91\%&69.65\%&85.00\%  \\
Network in Network&58.21\%&67.30\%&76.97\% \\ \midrule
\end{tabular}
\end{center}
\caption{Taking subsets of ImageNet. The gap between RFNNs and CNNs increases for fewer classes.}
\label{tab:imnetSubsets}
\end{table}


\begin{figure}
\includegraphics[width=0.5\textwidth, center]{mnist.eps}
\caption{Classification performance of the scattering network on various subsets of the MNIST dataset. In comparison the state of the art CNN-A from the literature on a subset of 300 samples. RFNN denotes our receptive field network, with the same architecture as CNN-B. Both are shown, to illustrate that good performance of the RFNN is not due to the CNN architecture, but due to RFNN decomposition. Our RFNN performs on par with Scattering, substantially outperforming CNN's on random MNIST subsets.}
\label{fig:MNIST}
\end{figure}


% The second part of the experiments is concerned with comparison to the scattering approach to show, that we outperform it on very small MNIST subsets as an example of very small non-natural image datasets where the scattering network has been shown to be state of the art~\cite{brunaTPAMI13scattering}, while we also perform better on the more challenging datasets Cifar-10/100, shown in [REF].
 
 
%We compare our approach to scattering networks on three datasets. We use multiple averaged runs on a tiny subset of MNIST to illustrate our ability to tackle small data non-natural image problems. On this problem scattering is de-facto state of the art. Furthermore we compare on two more challenging benchmarks, Cifar-10 and Cifar-100.

\subsection{Experiment 4: 3D Classification}

%We do two experiments on medical images, to show the value of our approach for images where pre-training doesn't work (2D Bone texture), or is simply not possible (3D Brain Scans).

 
We apply a RFNN to 3D brain scan classification for Alzheimer's~\cite{cuingnet2011automatic}, a domain where training data is notoriously small and no big open access databases in a similar domain exist for pre-training. \\

We use a 3 layer RFNiN, with a basis of order 10 in 3 scales $\sigma$=1,4,16. This time more extremely spaced, as the brains are always centered and have been normalized to MNI space with FSL library~\cite{jenkinson2012fsl}. Each basis layer is followed by one 1x1 convolution layer. Having 128 units in layer 1, 96 units in layer 2 and 64 units in layer 3. Global average pooling is applied to the final feature maps. The network has been implemented in the Theano library~\cite{bastien2012theano}.

The results are in Table~\ref{tab:brains}. We outperform the state-of-the-art, including a 3D CNN. The same 3 layer NiN as our RFNiN model does not converge on the dataset and gives random predictions. Thus we show our model is effective when data is scarce.


\begin{table}
\begin{center}
\begin{tabular}{@{}llll@{}}\toprule
Method&Accuracy&TPR&SPC\\ \midrule
%3D-RFNN A&99.32\%& &\\
3D-RFNiN (ours)&\textbf{97.79\%}& \textbf{97.14\%}& \textbf{98.78\%} \\
%3D-CNN A&98.79\%& &\\
%3D-CNN B&(Chance)\%& &\\
3D-CNN~\cite{DBLP:journals/corr/PayanM15}&95.70\%&-&-\\
NIB~\cite{gupta2013natural}&94.74\%&95.24\%&94.26\%\\
ICA~\cite{yang2011independent}&80.70\%&81.90\%&79.50\%\\
Voxel-Direct-D-gm~\cite{cuingnet2011automatic}&-&81.00\%&95.00\%\\ \midrule
3D-NiN (our baseline)&84.21\%& -\%& -\% \\
\midrule
\end{tabular}
\end{center}
\caption{Results on training with 150 brain MRI images of the ADNI standard benchmark. RFNNs outperform all published results. Reported is classification accuracy, true positive rate and specificity on the test set.}
\label{tab:brains}
\end{table}

\begin{table}
\begin{center}
\begin{tabular}{@{}llll@{}}\midrule
Method&Accuracy&EER\\ \midrule
3D-RFNiN (ours)&\textbf{87.67\%}& \textbf{-}& \textbf{-} \\
Local SVM~\cite{chen2014detecting}&74.10\%&-&-\\
FBM~\cite{toews2010feature}&-&70.00\%&-\\
Voxel-Direct-D-gm~\cite{cuingnet2011automatic}&-&-\%&-\%\\
\bottomrule
\end{tabular}
\end{center}
\caption{Results of training on the OASIS AD-126 dataset described in~\cite{toews2010feature}. Training has been done by .....}
\label{tab:brains}
\end{table}


%\begin{table}
%\begin{center}
%\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
%\hline
%RFNN based on NiN  \\
%Basis& 1x1Conv& ReLU& 1x1Conv& ReLU& MaxPool& Basis& 1x1Conv& ReLU& 1x1Conv& ReLU& MaxPool& Basis& 1x1Conv& ReLU& 1x1Conv& ReLU& MaxPool& Basis& 1x1Conv& ReLU& %1x1Conv& ReLU& Global Pool
%\hline
%\end{tabular}
%\end{center}
%\caption{RFNN architecture used}
%\end{table}


%\begin{table}
%\begin{center}
%\begin{tabular}{|l|l|}
%\hline
%Filters in Layer 1 & Top-1  \\%& Accuracy LR 0.01 \\
%\hline\hline
%Network in Network-96 & 56.85\% \\
%Network in Network-15 & 55.62\%  \\
%RFNN $1^{st}$-order & 54.16\% \\
%RFNN $2^{nd}$-order & 55.28\% \\
%RFNN $3^{rd}$-order & 57.60\% \\
%RFNN $4^{th}$-order & 70.22\%  \\
%\hline
%\end{tabular}
%\end{center}
%\caption{Shows orders for first layer basis. These results were trained with RMSprop due to the different learning rates necessary per layer.}
%\end{table}






%\begin{table}
%\begin{center}
%\begin{tabular}{@{}lll@{}}\toprule
%Method & Top-1 & \# of Parameters \\ \midrule
%RFNN scale=1 & running\% \\
%RFNN scale=2 & running\% \\
%RFNN scale=3 & ??\% \\
%RFNN scale=4 & ??\% \\  \bottomrule
%\end{tabular}
%\end{center}
%\caption{Table 1c RFNN with increased scale, up to scale 4 (5 if time). This affects all layers, as there is no reason for scale only to be extracted in layer 1, frequency decreasing paths can be ommited, thus higher layer have lesser sigmas -> 4*10h=50h}
%\end{table}





%\begin{table}
%\begin{center}
%\begin{tabular}{|l|c|c|c|}
%\hline
%Method & Top-1 & Top-5 \\
%\hline\hline
%RFNN  & \% & &\\
%Alexnet  & \% & &\\
%NiN  & \% & &\\
%\hline
%\end{tabular}
%\end{center}
%\caption{Full Imagenet}
%\end{table}







%\begin{figure}
%\includegraphics[width=0.5\textwidth, right]{filters_ordered_L1_beta.png}
%\caption{Effective filters learned by the network in Layer 1, ordered by highest energy per order and rotation. Higher scales are normalized for visualization by multiplying them with sigma. 
%\label{fig:filters}}
%\end{figure}






\end{document}

